The sound of my voice: speaker representation loss for target voice separation

Content and style representations have been widely studied in the field of style transfer. In this paper, we propose a new loss function using speaker content representation for audio source separation, and we call it speaker representation loss. The objective is to extract the target speaker voice from the noisy input and also remove it from the residual components. Compared to the conventional spectral reconstruction, our proposed framework maximizes the use of target speaker information by minimizing the distance between the speaker representations of reference and source separation output. We also propose triplet speaker representation loss as an additional criterion to remove the target speaker information from residual spectrogram output. VoiceFilter framework is adopted to evaluate source separation performance using the VCTK database, and we achieved improved performances compared to the baseline loss function without any additional network parameters.

==> TEMP.tex <==

\begin{table}[]
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{3}{|c|}{\begin{tabular}[c]{@{}c@{}}Noisy audio without VoiceFilter (Baseline) :\\ Mean SDR : 6.0092 {[}dB{]}, PESQ : 2.0586\end{tabular}}                                                               \\ \hline
                                                                                               & \begin{tabular}[c]{@{}c@{}}Mean SDR\\ Improv.\end{tabular} & \begin{tabular}[c]{@{}c@{}}PESQ\\ Improv.\end{tabular} \\ \hline
Conventional VoiceFilter{~\cite{wang2019interspeech}}                                                               & 4.1198                                                     & 0.4774                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}+ Content loss\\ (with reference audio)\end{tabular}                & 4.4363                                                     & 0.4953                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}+ Content loss \\ (with clean audio)\end{tabular}                   & 4.3542                                                     & 0.4952                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}+ Triplet content loss\\ (with reference audio anchor)\end{tabular} & 4.4727                                                     & 0.5005                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}+ Triplet content loss\\ (with clean audio anchor)\end{tabular}     & \textbf{4.6148}                                            & \textbf{0.5250}                                        \\ \hline
\end{tabular}
\caption{\textbf{PESQ and SDR improvements} compared to noisy audio baseline without VoiceFilter}
\end{table}

